Data Augmentation using Pre-trained Transformer Models

Language model based pre-trained models such as BERT have provided significant gains across different NLP tasks. In this paper, we study different types of transformer based pre-trained models such as auto-regressive models (GPT-2), auto-encoder models (BERT), and seq2seq models (BART) for conditional data augmentation. We show that prepending the class labels to text sequences provides a simple yet effective way to condition the pre-trained models for data augmentation. Additionally, on three classification benchmarks, pre-trained Seq2Seq model outperforms other data augmentation methods in a low-resource setting. Further, we explore how different pre-trained model based data augmentation differs in-terms of data diversity, and how well such methods preserve the class-label information.

==> sections/background.tex <==
\section{Data Augmentation for Text}
Data augmentation methods can be broadly categorized into three categories. 

\textbf{Context-Independent DA}: methods apply word level based transformation without considering other words in the example. For example, EDA~\cite{wei2019eda} proposed word replacement based data augmentation which replaces certain tokens with their synonyms to generate new examples. Since such methods does not take context into account, these methods do not guarantee that the generated data will be grammatically correct, meaningful. 
    
\textbf{Contextual DA}: Contextual augmentation approach for text data have been proposed ~\cite{zhu2019soft,kobayashi2018contextual}, in which a pre-trained LM is used to generate substitutions of words in a sentence. Such augmentation might not preserve the class labels as the model does not consider class while predicting the replacement tokens. Machine translation methods and Backtranslation~\cite{sennrich2015improving, xie2019unsupervised} are other contextual data augmentation which relies on having a good quality machine translation system.  
    
\textbf{Conditional DA}: ~\citet{wu2019conditional} proposed a contextual augmentation method in which a conditional BERT~\cite{devlin2018bert} LM is used to generate substitutions of words in a sentence. Similarly, ~\citet{anaby2019not} used a fine-tuned GPT2 model for conditional data augmentation. Since, such model condition generation on the class, they are more likely to preserve the label information during substitutions/generation. For text classification, conditional data augmentation performs better than contextual and context-independent methods. In this paper, we focus on exploring different conditional data augmentation methods.   




